Unbundle-Rewrite-Rebundle: Runtime Detection and Rewriting of Privacy-Harming Code in JavaScript Bundles

This work presents Unbundle-Rewrite-Rebundle (URR), a system for detecting privacy-harming portions of bundled JavaScript code and rewriting that code at runtime to remove the privacy-harming behavior without breaking the surrounding code or overall application. URR is a novel solution to the problem of JavaScript bundles, where websites pre-compile multiple code units into a single file, making it impossible for content filters and ad-blockers to differentiate between desired and unwanted resources. Where traditional content filtering tools rely on URLs, URR analyzes the code at the AST level, and replaces harmful AST sub-trees with privacy-and-functionality maintaining alternatives. We present an open-sourced implementation of URR as a Firefox extension and evaluate it against JavaScript bundles generated by the most popular bundling system (Webpack) deployed on the Tranco 10k. We evaluate URR by precision (1.00), recall (0.95), and speed (0.43s per script) when detecting and rewriting three representative privacy-harming libraries often included in JavaScript bundles, and find URR to be an effective approach to a large-and-growing blind spot unaddressed by current privacy tools.

==> 01-alt_intro_chris.tex <==
\section{Introduction}
An enormous body of research has established Web content filtering (e.g.,
blocking advertising and/or tracking related network requests on websites)
as an important and effective technique for improving privacy\cite{merzdovnik2017block, gervais2017quantifying}, security\cite{li2012knowing, zarras2014dark}, and performance\cite{garimella2017ad, pujol2015annoyed}. Most Web content filtering
approaches rely on crowd sourced lists of regular-expression-like rules that
describe which URLs the browser should load, and which should be blocked.

This approach---broadly, URL based content filtering---works because
URLs in practice provide useful information about the the resources they
map to. In some cases this is because of the text in the URL (e.g., browsers
can make a reasonable guess about the purpose of JavaScript returned from
a URL like\\
\texttt{https://advertising.example/tracker.js}), or because experts
have manually evaluated the resource returned from a URL and found it to
be similarly harmful to users.

However, modern Web development practices make content filtering difficult,
by combining multiple individual JavaScript code units into a single ``bundled''
code unit. Where sites might have previously included their Web application
as discrete, independently fetched JavaScript files, application developers
increasingly fetch each required JavaScript library at application build time,
package them into a single resource, and instead have users download and execute
a single, combined JavaScript file. In other words, web applications that
previously fetched three JavaScript files
(e.g., \texttt{/script/library.js}, \texttt{/script/tracker.js}, and
\texttt{/script/app.js}), are increasingly deployed by combining all
referenced code units into a single JavaScript resource (e.g., \texttt{/script/bundle.js}).

% There is a wide range of bundling techniques used on the Web. The most
% common kinds of JavaScript bundling are tools like
% Webpack\footnote{\url{https://webpack.js.org/}}, which bundle multiple JavaScript
% libraries into a single sources as part of a Node based build process.
% Google has proposed a similar approach called
% Web Bundles\footnote{\url{https://developer.chrome.com/docs/web-platform/web-bundles/}},
% which allow entire Web pages and their sub-resources (e.g., JavaScript, CSS, images)
% to be bundled into a single archive. And CDN companies like Cloudflare
% offer systems like ``Managed Components''\footnote{\url{https://managedcomponents.dev/}}
% that allow bundling-as-a-service at the network edge.

These bundling approaches, inadvertently or otherwise, circumvent
Web filter tools, because they combine resources that originally came from multiple, descriptive URLs,
into a large, bundled resource. To build on the example from two paragraphs earlier,
Web content filter tools previously could (for example) block \texttt{/script/tracker.js}
but still load \texttt{/script/library.js} and \texttt{/script/app.js}. But
when Web applications are delivered as single bundles, content filtering tools
can no longer easily block just parts of the application; blocking a web site's JavaScript  largely becomes an all-or-nothing proposition.

This work explores whether Web content filtering tools can continue
fine grained blocking decisions (i.e., omitting undesirable parts of a
Web application, while still loading other parts), even when Web
applications are delivered as monolithic Web bundles. This is an important,
practical research question for Web privacy, security, and performance; as
the popularity of ``bundled'' Web applications increases, the usefulness
of current URL based content filtering tools decreases. To return
to the example from previous paragraphs, we aim to allow browsers
to avoid executing the code from \texttt{/script/tracker.js}, while still
executing the non-privacy harming code originally provided in \texttt{/script/library.js}
and \texttt{/script/app.js}, \emph{even when} all three libraries are compiled
and delivered in \texttt{/script/bundle.js}. % a single Web bundle.

Such a system faces  several non-trivial challenges.

\textbf{First}, the
system must re-identify known-privacy harming code (e.g., the code originally
delivered from \texttt{/script/tracker.js}) within the larger bundled application,
in the absence of any information about the URL the code originally came from.
This problem is made even more difficult because popular bundling systems
post-process, minify, ``tree-shake'', and otherwise optimize each library
during the bundling process. As a result, code may change significantly
in both presentation (i.e., labels) and structure (i.e., top level functions,
classes, constants, etc) during the bundling process, making reidentification
difficult.

\textbf{Second}, even once a known-privacy-harming library has been identified
within a larger bundled application, a practical system must remove the harmful
(or otherwise undesired) code \emph{without breaking the surrounding code} that
expects the target library to be in place. Just deleting a unwanted libraries
from a bundled application will, in practice, be counter productive, since the
application will fail when trying to access now-deleted functions and classes
defined by the deleted library. A useful solution must remove the unwanted,
target libraries from the bundled application \emph{without breaking surrounding
code}.

\textbf{Third}, such a system must be performant, and be able to decompile,
analyze, modify, and recompile bundled Web applications quickly, in a way
that maintains the usefulness of the Web application. If the performance
overhead of a privacy-and-security preserving system is too costly, then the system
is in practice unusable, and so not meaningfully useful at benefit Web users.

This paper presents \system, a system dynamically blocking known-harmful JavaScript
code from bundled Web applications, without harming user-beneficial behaviors
in those Web applications. \system works by

\begin{itemize}
  \item offline building a database of signatures of the ASTs of top level
    structures in targeted (i.e., unwanted) JavasScript libraries
  \item modifying a commodity Web browser (via a Firefox browser extension) to
    identify and decompile bundled Web applications into their component modules/sub-libraries,
  \item searching for known-unwanted libraries in bundled
    application by generating signatures for each sub-module, and checking
    them against the offline generated database of known-unwanted code
  \item if a match is found, then replacing the target code with a pre-authored
    compatibility-maintaining shim implementation of the target library,
    and then passing the the now-modified bundled application to the
    browser's JavaScript engine.
\end{itemize}

\subsection{Contributions}
Specifically, this work makes the following contributions to the area
of Web privacy and security.

\begin{enumerate}
  % \item An empirical Web measurement of bundled JavaScript applications,
  %   showing that current Web content filtering tools have a false positive
  %   rate when dealing with bundled Web applications (i.e., bundling
  %   causes Web content filtering tools to load libraries that would otherwise
  %   be blocked in X\% of cases).
  \item A novel algorithm for efficiently generating fingerprints of
    top-level structures in JavaScript libraries. These fingerprints are
    robust to many of the modifications that bundling tools make during
    their complication process (e.g., label minification, ``tree-shaking'').
  \item An open sourced, empirically tuned system for
    \begin{enumerate}
      \item decompiling bundled applications into their constant libraries
      \item generating fingerprints for each sub-library and checking
        them against a database of known unwanted JavaScript libraries
      \item replacing unwanted JavaScript libraries with compatibility-preserving
        ``shim'' implementations, which maintain the library's API ``shape'',
        while removing any privacy-or-security affecting behaviors
      \item recompiling the resulting new application into a new bundle, that
        can then be passed to the browser's JavaScript engine for normal
        execution.
    \end{enumerate}
  \item An empirical evaluation of the accuracy and performance of our
    system when applied to a representative crawl of the Web, finding
    that our system results in libraries being blocked on 7\% of the top 10K sites in the Tranco list, within practical performance bounds.
  \item An open source implementation of our system as a Firefox extension,
    along with the complete dataset for all discussed figures and measurements.
  \end{enumerate}

==> 01-introduction.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
\label{sec:introduction}
%-------------------------------------------------------------------------------

In recent years, the pervasive nature of online tracking has emerged as a critical concern in the realm of internet privacy. With a growing awareness of these privacy intrusions, extension authors and browser vendors have taken significant steps to mitigate such tracking practices. Trackers have continually evolved to circumvent these mitigations as these restrictions become more widespread.

One such method of circumvention involves the use of bundlers. In modern web development, bundlers are a general-use tool that aggregates dependencies for deployment across diverse platforms. Historically, tracking libraries and many other plug-and-play libraries have been individually included as stand-alone JavaScript libraries. As such, many traditional techniques like pattern matching over the URL or the file body could effectively neutralize these tracking libraries. However, modern websites increasingly include tracking libraries within their full bundled website functionality. Because bundlers commingle non-tracking and tracking functionality within the same individual JavaScript file, these traditional techniques can neither effectively detect nor neutralize this embedded tracking functionality.  As this practice becomes increasingly prevalent, there is an urgent need for effective countermeasures.

In response to this emerging threat, this paper introduces a novel static analysis framework to tackle bundled tracking code. It methodically identifies bundled packages, deconstructs them to isolate individual modules, and then scrutinizes these modules for tracking code. Upon detecting tracking elements, our system replaces these intrusive modules with benign counterparts. After this cleansing process, the framework reassembles the packages and safely reintroduces them to the website, ensuring functionality while enhancing privacy.

To validate the efficacy of our framework, we conducted extensive evaluations using three widely-used library bundles. Our results demonstrate the framework's effectiveness in detecting and neutralizing trackers on popular websites and its practicality, as evidenced by performance measurements. These findings underscore the potential of our framework as a pivotal tool in the ongoing battle against online tracking, offering a new avenue for safeguarding user privacy in an increasingly interconnected digital world.

\iffalse

[paragraph1] Tracking has been a problem. Browser vendors are cracking down on it.

[paragraph2] Trackers are finding ways of getting around restrictions placed on third-party code.

[paragraph3] Bundlers help gather dependencies in large codebases and run them on multiple platforms. They are difficult to break apart.

[paragraph4] Trackers can evade detection by hiding in bundlers. With this practice growing more common, we need solutions.

[paragraph 5] We present a static analysis framework that identifies bundles, breaks them apart, identifies individual modules, replaces tracker modules with benign code, stitches them back up, and sends them to the website.

[paragraph6] We evaluate our framework against 3 popular libraries. We show its effectiveness on popular sites and its practical use through performance measurements.

\fi

\subsection{Contributions}

\begin{itemize}
    \item New Generic framework
    \item Demonstrate implementation using webpack
    \item Demonstrated detection of three popular libraries.
    \item Measurements and evaluation
    \item Open source implementation
\end{itemize}

==> 08-artifact.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Artifact Appendix Template for ACM CCS 2024.
% See end of this file for authorship and provenance info.
%
% Please limit your Artifact Appendix to no more than two pages.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% This template uses list-making environments from the `paralist`
%% LaTeX package.  Add the following to the preamble of your LaTeX
%% document (somewhere before `\begin{document}`:
%%
%% \usepackage{paralist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \appendix

\section{Artifact Appendix}

\emph{The Artifact Appendix is meant to summarize the purpose,
availability, content, dependencies, and execution of the artifacts
that support your paper.  It should include a clear description of
your artifacts' hardware, software, and configuration requirements.
If your artifacts have received the \emph{Artifacts
Evaluated--Functional}, \emph{Artifacts Evaluated--Reusable}, or
\emph{Results Reproduced} badge, this appendix should summarize the
relevant major claims made by your paper and provide instructions for
validating each claim through the use of your artifacts.  Linking the
claims of your paper to the artifacts allows a reader of your paper
to more easily try to reproduce your paper's results.}

\emph{Please fill in all the mandatory sections, keeping their titles
and organization but removing the current illustrative content, and
remove the optional sections that do not apply to your artifacts.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Abstract}

\emph{[Mandatory]}
%
\emph{Provide a short description of your artifacts.  What do they
contain?  How are they packaged?  What do they do when executed?  What
results to they produce?  How are your artifacts licensed?  Be brief;
subsequent sections of this appendix can be used fill in the details.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Description \& Requirements}

\emph{This section should further detail your artifacts and summarize
the requirements that must be met for a person to recreate an
experimental environment for utilizing your artifacts.  Where
applicable, state the minimum hardware and software requirements for
running your artifacts.  It is also good practice to list and describe
in this section benchmarks where those are part of, or simply have
been used to produce results with, your artifacts.}

\emph{[Mandatory]}
%
\emph{Here, provide additional details about the general organization
of your artifacts.  For example, provide a general roadmap to the
files within your artifacts.  Where is the \texttt{README}?  Where are
the source files, the datasets, the scripts for running experiments,
etc.?  You don't need to describe every file and directory here; just
provide a general ``lay of the land.''}

%%%%%

\subsubsection{Security, privacy, and ethical concerns}

\emph{[Mandatory]}
%
\emph{Describe any risks that people might be exposed to while
executing your artifacts: e.g., risks to their machines' security,
data privacy, or other ethical concerns.  This is particularly
important if destructive steps are taken or security mechanisms are
disabled during execution.}

%%%%%

\subsubsection{How to access}

\emph{[Mandatory]}
%
\emph{Describe how to access your artifacts.  If your artifacts have
received the \emph{Artifacts Available} badge, you must provide the
DOI(s) for the permanently and publicly available copies of your
artifacts.  Most likely, this is the version of your artifacts that
you deposited with Zenodo.}

\emph{You may describe more than one way to access your artifacts.
For example, if the archived versions of your artifacts are available
at Zenodo, and you are also making maintained versions of your
artifacts available through GitHub, you can describe how to access
both versions of your artifacts.}

%%%%%

\subsubsection{Hardware dependencies}

\emph{[Mandatory]}
%
\emph{State any specific hardware features that are required to make
use of your artifacts: e.g., vendor, CPU/GPU/FPGA, number of
processors/cores, microarchitecture, interconnect, memory, hardware
counters, etc.  If your artifacts do not have significant hardware
dependencies, simply write ``None'' in this section.}

%%%%%

\subsubsection{Software dependencies}

\emph{[Mandatory]}
%
\emph{State any specific OS and software packages that are required to
make use of your artifacts.  This is particularly important if you
share your source code and it must be compiled, or if your artifacts
rely on proprietary software that is not included in your artifact
packages.  If your artifacts do not have significant software
dependencies, simply write ``None'' in this section.}

%%%%%

\subsubsection{Benchmarks}

\emph{[Mandatory]}
%
\emph{Describe any data (e.g., datasets, models, workloads,
etc.)\ required by the experiments that are reported in your paper and
supported by your artifacts.  If this does not apply to your
artifacts, simply write ``None'' in this section.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Set Up}

\emph{This section should summarize the installation and configuration
steps that a person should follow to prepare an environment for making
use of your artifacts.  If the set-up steps are complicated, point the
reader to the places in your artifacts where detailed set-up
instructions can be found.}

%%%%%

\subsubsection{Installation}

\emph{[Mandatory]}
%
\emph{Provide instructions for downloading and installing dependencies
as well as the main artifacts.  After following these steps, a user of
your artifacts should be able to run a simple functionality test.}

%%%%%

\subsubsection{Basic test}

\emph{[Mandatory]}
%
\emph{Provide instructions for running a simple functionality test.
This test does not need to exercise all the features of your
artifacts, but ideally, it should allow a user to check that all of
the required software components are correctly installed and
functioning as intended.  Please include the expected successful
output and any required input parameters.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Evaluation Workflow}

\emph{This section should include all the operational steps and
experiments that a person must be carry out to utilize in your
artifacts toward the goal of validating your paper's key results and
claims.  To that end, we ask you to use the two following subsections
and cross-reference the items therein as explained below.}

%%%%%

\subsubsection{Major claims}

\emph{[Mandatory for \emph{Artifacts Evaluated--Functional},
  \emph{Artifacts Evaluated--Reusable}, and \emph{Results Reproduced};
  optional for \emph{Artifacts Available}]}
%
\emph{Enumerate here the major claims (Cx) made in your paper.  Follow
the examples below.}
% \bigskip

% \begin{compactitem}
\begin{itemize}[nosep,noitemsep]
\item[(C1):]
  %
  \emph{System\_name achieves the same accuracy as the
  state-of-the-art systems for a task X while requiring Y\% less
  storage.  This is proven by the experiment (E1) described in [refer
    to your paper's sections], whose results are illustrated/reported
  in [refer to your paper's plots, tables, sections, etc.].}

\item[(C2):]
  %
  \emph{System\_name has been used to uncover new bugs in the X
  software.  This is proven by experiments (E2) and (E3) in [refer to
    your paper's sections].}
% \end{compactitem}
\end{itemize}

%%%%%

\subsubsection{Experiments}

\emph{[Mandatory for \emph{Artifacts Evaluated--Functional},
  \emph{Artifacts Evaluated--Reusable}, and \emph{Results Reproduced};
  optional for \emph{Artifacts Available}]}
%
\emph{Explicitly link the descriptions of your experiments to the
items you have provided in the previous subsection about major claims.
Please provide estimates of the person- and compute-time required for
each of the listed experiments (using the suggested hardware/software
configuration).  Follow the examples below.}

% \bigskip
% \begin{compactitem}
\begin{itemize}[nosep,noitemsep]
\item [(E1):]
  %
  \emph{[Optional Name] [30~person-minutes + 1~compute-hour + 5\,GB
    disk]: Provide a short explanation of the experiment and expected
  results.}

  \emph{Provide the steps to perform the experiment and collect and
  organize the results as expected from your paper.  We encourage you
  to use the following structure with three main blocks for the
  description of your experiment.  If the procedures are complicated,
  point the reader to the places in your artifacts where the full
  instructions can be found.}
  
  % \begin{asparadesc}
  \textbf{Preparation:} \emph{Describe the steps required to prepare and
  configure the environment for this experiment.}

  \textbf{Execution:} \emph{Describe the steps required to run this
  experiment.}

  \textbf{Results:} \emph{Describe the steps required to collect and
  interpret the results for this experiment.}
  % \end{asparadesc}

\item[(E2):] \emph{[Optional Name] [1~person-hour + 3~compute-hours]: \ldots}

\item[(E3):] \emph{[Optional Name] [1~person-hour + 3~compute-hours]: \ldots}
% \end{compactitem}
\end{itemize}
% \bigskip

\emph{In all of the above blocks, please provide indications about the
expected outcome for each of the steps (given the suggested hardware
and software configuration).}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Notes on Reusability}

\emph{[Optional]}
%
\emph{This section is meant to provide additional information about
how a person could utilize your artifacts beyond the research
presented in your paper.  A broad objective of artifact evaluation is
to encourage you to make your research artifacts reusable by others.}

\emph{Include in this section any instructions, guidance, or advice
that you believe would help others reuse your artifacts.  For example,
you could describe how one might scale certain components of your
artifacts up or down; apply your artifacts to different kinds of
inputs or datasets; customize your artifacts' behavior by replacing
specific modules or algorithms; etc.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Version}
%%%%%%%%%%%%%%%%%%%%
% Obligatory.
% Do not change/remove.
%%%%%%%%%%%%%%%%%%%%
Based on the LaTeX template for Artifact Evaluation V20220926.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% AUTHORSHIP AND PROVENANCE OF THIS TEMPLATE

%% This template was created by Eric Eide for the ACM CCS 2024
%% conference.
%%
%% The AEC Chair for CCS 2024 was:
%% Eric Eide (University of Utah)

%% This template is based on the "USENIX Security 2023 AE Template."
%% https://secartifacts.github.io/usenixsec2023/appendix/usesec23-ae-latex.zip
%%
%% The AEC Co-chairs for USENIX Security 2023 were:
%% Cristiano Giuffrida (Vrije Universiteit Amsterdam)
%% Anjo Vahldiek-Oberwagner (Intel Labs)

%% The USENIX Security AE template was based on the
%% % Artifact Appendix Template for EuroSys'22 AE
%% https://sysartifacts.github.io/eurosys2022/appendix/EuroSys22_ArtifactAppendix_template.tex
%%
%% The AEC Co-chairs for EuroSys 2022 were:
%% Natacha Crooks (UC Berkeley)
%% Solal Pirelli (EPFL)
%% Salvatore Signorello (University of Lisbon)
%% Anjo Vahldiek-Oberwagner (Intel Labs)

%% The above were based on:

%% LaTeX template for Artifact Evaluation V20220119
%%
%% Original Authors
%% * Grigori Fursin (cTuning foundation, France) 2014-2020
%% * Bruce Childers (University of Pittsburgh, USA) 2014
%%
%% Modified by
%% * Clementine Maurice (CNRS, France) 2021-2022
%% * Cristiano Giuffrida (Vrije Universiteit Amsterdam, Netherlands) 2021-2022
%%
%% (C) Copyright 2014-2022
%%
%% CC BY 4.0 license
%%

